Optical coherence and spin population dynamics in $^{171}$Yb$^{3+}$:Y$_2$SiO$_5$ single crystals

$^{171}$Yb$^{3+}$-doped Y$_2$SiO$_5$ crystals are a promising platform for optical quantum memories in long-distance quantum communications. The relevance of this material lies in $^{171}$Yb long optical and spin coherence times, along with a large hyperfine splitting, enabling long quantum storage over large bandwidths. Mechanisms affecting the optical decoherence are however not precisely known, especially since low-temperature measurements have so far focused on the 2 to 4 K range. In this work, we performed two- and three-pulse photon echoes and spectral hole burning to determine optical homogeneous linewidths in two 171 Yb:YSO crystals doped at 2 and 10 ppm. Experiments were performed in the 40 mK to 18 K temperature range, leading to linewidths between 320 Hz, among the narrowest reported for rare-earth ions, and several MHz. Our results show that above 6 K the homogeneous linewidth is mainly due to an elastic two-phonon process which results in a slow broadening with temperature, the homogeneous linewidth reaching only 25 kHz at 10 K. At lower temperatures, interactions with $^{89}$Yb nuclear spin-flips, paramagnetic defects or impurities, and also Yb-Yb interactions for the higher concentrated crystal, are likely the main limiting factor to the homogeneous linewidth. In particular, we conclude that the direct effect of spin and optical excited state lifetime is a minor contribution to optical decoherence in the whole temperature range studied. Our results indicate possible paths and regimes for further decreasing the homogeneous linewidths or maintaining narrow lines at higher $^{171}$Yb concentration.

==> xx.tex <==



==> yy.tex <==


